MedBN: Robust Test-Time Adaptation against Malicious Test Samples

Test-time adaptation (TTA) has emerged as a promising solution to address performance decay due to unforeseen distribution shifts between training and test data. While recent TTA methods excel in adapting to test data variations, such adaptability exposes a model to vulnerability against malicious examples, an aspect that has received limited attention. Previous studies have uncovered security vulnerabilities within TTA even when a small proportion of the test batch is maliciously manipulated. In response to the emerging threat, we propose median batch normalization (MedBN), leveraging the robustness of the median for statistics estimation within the batch normalization layer during test-time inference. Our method is algorithm-agnostic, thus allowing seamless integration with existing TTA frameworks. Our experimental results on benchmark datasets, including CIFAR10-C, CIFAR100-C and ImageNet-C, consistently demonstrate that MedBN outperforms existing approaches in maintaining robust performance across different attack scenarios, encompassing both instant and cumulative attacks. Through extensive experiments, we show that our approach sustains the performance even in the absence of attacks, achieving a practical balance between robustness and performance.

==> contents/proof.tex <==
% \section{Proof}
\subsection{Mean vs. Median}
We provide a simple analysis, demonstrating the robustness of using median instead of mean.
To do so, consider a set of $n$ numbers $X = \{x_i \in \mathbb{R}: i = 1,..., n\}$ where the first $m$ numbers are possibly manipulated by attackers and the others are drawn from a certain distribution.
Denoting $X_\textrm{mal} := \{x_i : i = 1,...,m\}$ and $X_\textrm{ben} := \{x_i : i = m+1,...,n\}$,


% Define medians:
% $\eta(X_\textrm{mal})$
% $\eta(X_\textrm{ben})$
% $\eta (X_\textrm{mal}\cup X_\textrm{ben})$

% Define means:
% $\mu(X_\textrm{mal})$
% $\mu(X_\textrm{ben})$
% $\mu(X_\textrm{mal}\cup X_\textrm{ben})$

For a finite set $A \subset \mathbb{R}$, denote
the mean and median of $A$ by
\begin{align}
\mu(A) &= \textrm{mean} (A)
= \frac{1}{|A|} \sum_{a \in A} a \;, \text{and} \\
 \eta(A) &= \textrm{median} (A)
= \min_{a \in A : |\{x \in A: a  > x\}|\ge \frac{|A|}{2}} a \;.
\end{align}

\begin{align}
\max_{X_\textrm{mal}} |
\eta(X_\textrm{mal}\cup X_\textrm{ben})
-\eta(X_\textrm{ben})
| \le 
\frac{}{} \max_{x, x' \in X_\textrm{ben}}
|x - x'| < 
\infty
\end{align}


\begin{align}
\max_{X_\textrm{mal}} |
\eta(X_\textrm{mal}\cup X_\textrm{ben})
-\mu(X_\textrm{ben})
| < \infty
\end{align}


\begin{align}
\max_{X_\textrm{mal}} |
\eta(X_\textrm{mal}\cup X_\textrm{ben})
- \mu(X_\textrm{ben})
| = \infty
\end{align}


\begin{align}
\max_{X_\textrm{mal}} |\mu_\textrm{ben} - \mu_\textrm{all}| = \infty
\end{align}



We analytically compare the mean and median.

To do so, 
we focus on 
estimating the mean of benign samples
given a test batch $\gB = \gB_{ben} \cup
\gB_{mal}$
consisting of benign and malicious samples. 





the e

a set of $X=\{x_1, \dots, x_m\}$, where $x_i \in \sR$. \\
If $n<\frac{m}{2}$, then for any subset $S \subseteq X$ with $|S|=m-n$, \\
we obtain that
\begin{align*}
    |\{ i \in S | x_i \leq \texttt{med}(x_1, ..., x_m)\}| \geq 
    \frac{m}{2} - n
    \quad and \\
    |\{ i \in S | x_i \geq \texttt{med}(x_1, ..., x_m)\}| \geq 
    \frac{m}{2} - n
\end{align*}



1. The same convergence on benign batches.


2. The vulnerability of mean on malicious batches.



3. The robustness of median on malicious batches.

\begin{theorem}
Th
\end{theorem}

\vspace{10em}




% \subsection{Theorem2}
% For $n<\frac{m}{2}$, 
% \begin{equation*}
%     || \tilde{x}_{i,B}^{(k)} - \hat{x}_{i,S}^{(k)}  || \leq
%     || \hat{x}_{i,B}^{(k)} - \hat{x}_{i,S}^{(k)}  ||
% \end{equation*}



\iffalse 
%\subsection{Theoretical Analysis  of BA-TTA}
%\subsubsection{Lemma1}
\noindent 
Consider a set of $X=\{x_1, \dots, x_m\}$, where $x_i$ $\in$ $\realnum$. \\
If $n<\frac{m}{2}$, then for any subset $S \subseteq X$ with $|S|=m-n$, \\
we obtain that
\begin{align*}
    |\{ i \in S | x_i \leq \texttt{med}(x_1, ..., x_m)\}| \geq 
    \frac{m}{2} - n
    \quad and \\
    |\{ i \in S | x_i \geq \texttt{med}(x_1, ..., x_m)\}| \geq 
    \frac{m}{2} - n
\end{align*}

\paragraph{Proof}
Proof can be found in Appendix.

\subsubsection{Theorem1}
\noindent
Consider a batch $B={\{x_1, \dots, x_m}\}$ \\
For $n<\frac{m}{2}$, 
\begin{equation*}
    | \mu_{S}^{(k)} - \eta_{B}^{(k)}  | \leq
    \frac{m}{2(m-n)}\underset{i, j \in S}{\max}(x_i^{(k)} - x_j^{(k)})
\end{equation*}

\paragraph{Proof}
Proof is similar to \cite{farhadkhani2022byzantine}.

\SP{



}

\vspace{10em}

\fi


% \subsection{Theorem2}
% For $n<\frac{m}{2}$, 
% \begin{equation*}
%     || \tilde{x}_{i,B}^{(k)} - \hat{x}_{i,S}^{(k)}  || \leq
%     || \hat{x}_{i,B}^{(k)} - \hat{x}_{i,S}^{(k)}  ||
% \end{equation*}



